Interactive Segmentation as Gaussian Process Classification

Click-based interactive segmentation (IS) aims to extract the target objects under user interaction. For this task, most of the current deep learning (DL)-based methods mainly follow the general pipelines of semantic segmentation. Albeit achieving promising performance, they do not fully and explicitly utilize and propagate the click information, inevitably leading to unsatisfactory segmentation results, even at clicked points. Against this issue, in this paper, we propose to formulate the IS task as a Gaussian process (GP)-based pixel-wise binary classification model on each image. To solve this model, we utilize amortized variational inference to approximate the intractable GP posterior in a data-driven manner and then decouple the approximated GP posterior into double space forms for efficient sampling with linear complexity. Then, we correspondingly construct a GP classification framework, named GPCIS, which is integrated with the deep kernel learning mechanism for more flexibility. The main specificities of the proposed GPCIS lie in: 1) Under the explicit guidance of the derived GP posterior, the information contained in clicks can be finely propagated to the entire image and then boost the segmentation; 2) The accuracy of predictions at clicks has good theoretical support. These merits of GPCIS as well as its good generality and high efficiency are substantiated by comprehensive experiments on several benchmarks, as compared with representative methods both quantitatively and qualitatively.

==> misc/fig_clicktime.tex <==
\begin{figure}[t]
  \centering
\includegraphics[width=0.98\linewidth]{figures/clicktime.pdf}
  \vspace{-0.4cm}
  \caption{Change of inference time with the click index, with Resnet50 as the backbone segmentor. The y-axis is in the log scale.}
\label{fig:clicktime}
  \vspace{-0.5cm}
\end{figure}


==> misc/tab_complexity2.tex <==
\begin{table}[t] 
\footnotesize
\caption{Model complexity and inference efficiency analysis where ResNet50 is adopted as the backbone segmentor. \vspace{-2mm}}
\label{tab:comp}
\centering
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{1.4mm}{
\begin{NiceTabular}[colortbl-like]{@{}l|c|c|cc@{}}
\toprule \multicolumn{1}{c}{\multirow{2}{*}{Method}} &
\multicolumn{1}{c}{\multirow{2}{*}{FLOPs (G)}} & \multicolumn{1}{c}{\multirow{2}{*}{\#Params (MB)}} & \multicolumn{2}{c}{SPC (ms)}   \\
 & & & GrabCut & DAVIS \\ \midrule
   RGB-BRS & 211.18  &  39.44 & 332.97 & 1104.04  \\
  f-BRS-B & 211.18 & 39.44  & 75.01 & 116.53  \\
   CDNet & 198.57 & 39.90 & 55.19 &  57.76 \\
 RITM & 98.86 & 39.48 & 31.82 &  34.24 \\
 % FocusCut & (\#Click+1)*\textcolor{black}{39.4} & 40.36 & 474.22  & 950.68 \\
 FocalClick & 99.24 & 39.50 & 37.64 & 41.80 \\
 \rowcolor{gray!20} GPCIS (Ours)   & 99.80 & 39.39 & 35.54 & 38.82 \\ 
 \bottomrule
\end{NiceTabular}}
\vspace{-5mm}
\end{table}


==> misc/tab_experiment2.tex <==
\begin{table*}[t] 
\footnotesize
% \caption{Evaluation results of NoC@85/90 on four classic datasets. `*' denotes the models trained on the Augmented PASCAL VOC dataset \cite{everingham2010pascal,hariharan2011semantic}, while other models are trained on the training split of the SBD dataset \cite{hariharan2011semantic}, which is a subset of the former training dataset. \vspace{-2mm}}


\caption{NoC@85 and NoC@90 of different competing methods on four datasets, \emph{i.e.}, GrabCut, Berkeley, SBD, and DAVIS. `*' denotes the models trained on the Augmented PASCAL VOC dataset \cite{everingham2010pascal,hariharan2011semantic}.}\vspace{-2mm}

\label{tab:exp}
\centering
\renewcommand{\arraystretch}{0.7}
\setlength{\tabcolsep}{0.7mm}{
\begin{NiceTabular}[colortbl-like]{@{}c|l|cc|cc|cc|cc|cc@{}}
\toprule \multicolumn{1}{c}{\multirow{2}{*}{Backbone}} &
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{GrabCut \cite{rother2004grabcut}} & \multicolumn{2}{c}{Berkeley \cite{mcguinness2010comparative}} & \multicolumn{2}{c}{SBD \cite{hariharan2011semantic}} & \multicolumn{2}{c}{DAVIS \cite{perazzi2016benchmark} } & \multicolumn{2}{c}{Average}   \\
& & NoC@85   & NoC@90 & NoC@85 & NoC@90   & NoC@85   & NoC@90 & NoC@85  & NoC@90 & NoC@85 & NoC@90  \\ 
\midrule
 \multicolumn{1}{c}{\multirow{5}{*}{ N/A}}  & GC \cite{boykov2001interactive} & 7.98 & 10.00 & - & 14.33 & 13.60 & 15.96 & 15.13 & 17.41 & - & 14.40 \\
  & GM \cite{bai2009geodesic} & 13.32 & 14.57 & - & 15.96 & 15.36 & 17.60 & 18.59 & 19.50 & - & 16.91 \\
  & RW \cite{grady2006random} & 11.36 & 13.77 & - & 14.02 & 12.22 & 15.04 & 16.71 & 18.31 & - & 15.29 \\
  & ESC \cite{gulshan2010geodesic} & 7.24 & 9.20 & - & 12.11 & 12.21 & 14.86 & 15.41 & 17.70 &  - &13.47 \\ 
    & GSC \cite{gulshan2010geodesic} & 7.10 & 9.12 & - & 12.57 & 12.69 & 15.31 & 15.35 & 17.52 & - & 13.63 \\ \midrule
DeepLab-LargeFOV \cite{chen2017deeplab} & RIS-Net \cite{liew2017regional} $^*$ & - & 5.00 & - &  6.03 & - & - & - & -  &- & - \\ \midrule
CAN \cite{YuKoltun2016} & LD \cite{li2018interactive} & 3.20 & 4.79 & - & - & 7.41 & 10.78 & 5.95 & 9.57 &- & - \\ \midrule
 \multicolumn{1}{c}{\multirow{2}{*}{FCN \cite{long2015fully}}} & DOS w/ GC \cite{xu2016deep} $^*$ & 5.08 & 6.08 & - & - & 9.22 & 12.80 & 9.03 & 12.58 &- & - \\
 & CMG \cite{majumder2019content} $^*$ & - & 3.58 & - & 5.60 & - & - & - & - &- & - \\ \midrule
DenseNet \cite{huang2017densely} & BRS \cite{jang2019interactive}& 2.60 & 3.60 & - & 5.08 & 6.59 & 9.78 & 5.58 & 8.24 &- & 6.68 \\ \midrule
Xception-65 \cite{chollet2017xception}& CA 
\cite{kontogianni2020continuous}  $^*$ & - & 3.07 & - & 4.94 & - & - & 5.16 & - &- & - \\ \midrule
 \multicolumn{1}{c}{\multirow{3}{*}{SegFormerB0-S2 \cite{xie2021segformer,chen2022focalclick}}} &
% FocusCut \cite{lin2022focuscut} & 1.92 & 2.62 & 5.42 & 5.06 & 7.64 & 6.21 & 9.65 & 6.33  \\
RITM \cite{sofiiuk2021reviving} & \textbf{1.62} & 1.82 & 1.84 & 2.92 & 4.26 & 6.38 & 4.65 & 6.13 & 3.09 & 4.31 \\
 & FocalClick \cite{chen2022focalclick} & 1.66 & 1.90 & - & 3.14 & 4.34 & 6.51 & 5.02 & 7.06 & - & 4.65  \\
% 216_GP_Segformer_SBD_click3_cs256_sota_L256_kernel9_normal_uloss2_sample_230epo
 &\cellcolor{gray!20} GPCIS (Ours)      &\cellcolor{gray!20} \textbf{1.62}  &\cellcolor{gray!20} \textbf{1.76} & \cellcolor{gray!20} \textbf{1.82} &\cellcolor{gray!20} \textbf{2.69} &\cellcolor{gray!20} \textbf{4.15} &\cellcolor{gray!20} \textbf{6.28} &\cellcolor{gray!20} \textbf{4.45} &\cellcolor{gray!20} \textbf{6.06}   &\cellcolor{gray!20} \textbf{3.01} &\cellcolor{gray!20} \textbf{4.20}  \\ \midrule
 \multicolumn{1}{c}{\multirow{3}{*}{HRNet18s-S2 \cite{wang2020deep,chen2022focalclick}}} & 
% FocusCut \cite{lin2022focuscut} & \textbf{1.52} & \textbf{1.72} & 3.69 & \textbf{3.80} & \textbf{5.93} & 5.05 & 7.38 & 4.68  \\
RITM \cite{sofiiuk2021reviving} & 2.00 & 2.24 & 2.13 & 3.19 & 4.29 & 6.36 & 4.89 & 6.54 & 3.33 & 4.58 \\
 & FocalClick \cite{chen2022focalclick} & 1.86 & 2.06 & - & 3.14 & 4.30 & 6.52 & 4.92 & 6.48 &-& 4.55  \\
% 054_GP_HRNetocr_SBD_click3_cs256_128_kernel9_normal_uloss2_detach_lr00005_230epo
 &\cellcolor{gray!20} GPCIS (Ours)     &\cellcolor{gray!20} \textbf{1.74} & \cellcolor{gray!20} \textbf{1.96} & \cellcolor{gray!20} \textbf{1.84} &\cellcolor{gray!20} \textbf{2.64} &\cellcolor{gray!20} \textbf{4.28} &\cellcolor{gray!20} \textbf{6.26} &\cellcolor{gray!20} \textbf{4.61} &\cellcolor{gray!20} \textbf{6.16}     & \cellcolor{gray!20} \textbf{3.12} &\cellcolor{gray!20} \textbf{4.26}  \\ \midrule
 \multicolumn{1}{c}{\multirow{7}{*}{ResNet50 \cite{he2016deep}}} 
  & FCANet\cite{lin2020interactive} $^*$    & 2.18 & 2.62 & - & 4.66 & - & - & 5.54 & 8.83 & -& -  \\
 & RGB-BRS \cite{sofiiuk2020f}   & 2.16 & 2.56 & 2.17 & 4.27 & 4.00 & 6.59 & 5.27 & 7.51 &3.40 & 5.23  \\
  & f-BRS-B \cite{sofiiuk2020f}   & 2.20 & 2.64 & 2.17 & 4.22 & 4.55 & 7.45 & 5.44 & 7.81 & 3.59 & 5.53  \\
 & CDNet \cite{chen2021conditional}   & 2.22 & 2.64 & - & 3.69 & 4.37 & 7.87 & 5.17 & 6.66 &-& 5.22  \\
& RITM \cite{sofiiuk2021reviving}  & 2.16 & 2.30 & 1.90 & 2.95 & 3.97 & 5.92 & 4.56 & 6.05 &3.15& 4.31  \\
% & FocusCut \cite{lin2022focuscut}   & \textbf{1.60} & \textbf{1.78} & 1.86 & 3.44 & \textbf{3.62}  & \textbf{5.66} & 5.00 & 6.38 &3.02& 4.32  \\
& FocalClick \cite{chen2022focalclick}   & 1.92 & 2.14 & 1.87 & 2.86 & 3.84 & 5.82 & 4.61 & 6.01 &3.06& 4.21   \\
% 299_GP_Resnet50_SBD_click3_cs256_ft48im_L256_kernel9_normal_uloss2_detach_230epo
 & \cellcolor{gray!20} GPCIS (Ours)  &\cellcolor{gray!20} \textbf{1.64} &\cellcolor{gray!20} \textbf{1.78} & \cellcolor{gr\textbf{}ay!20} \textbf{1.63} &\cellcolor{gray!20} \textbf{2.56} &\cellcolor{gray!20} \textbf{3.79} &\cellcolor{gray!20} \textbf{5.71} & \cellcolor{gray!20}\textbf{4.37} &\cellcolor{gray!20} \textbf{5.88}  & \cellcolor{gray!20} \textbf{2.86} & \cellcolor{gray!20} \textbf{3.98} \\ \bottomrule
\end{NiceTabular}}
\vspace{-4mm}
\end{table*}


==> misc/tab_metrics.tex <==
% \begin{table*}[t] 
% \small
% \caption{Metrics. \vspace{-3mm}}
% \label{tab:metrics}
% \centering
% \renewcommand{\arraystretch}{1.0}
% \setlength{\tabcolsep}{1.6mm}{
% \begin{NiceTabular}[colortbl-like]{@{}l|cccc|cccc@{}}
% \toprule \multicolumn{1}{c}{\multirow{2}{*}{Method}} &
% \multicolumn{4}{c}{Berkeley} & \multicolumn{4}{c}{DAVIS}    \\
%  & NoC$_{100}$@90 & NoF$_{100}$@90 & IoU\&1 & IoU\&5  & NoC$_{100}$@90 & NoF$_{100}$@90 & IoU\&1 & IoU\&5  \\ \midrule
%   f-BRS-B & 6.21 & 2 & 77.06\% & 85.00\%  & 22.62 & 57 & 70.97\% & 83.87\%    \\
%  RITM & 3.75 & \textbf{1} & 76.88\% & 94.66\%  & 18.09 & 51 & 72.89\%  & 89.14\% \\
%  FocusCut & 4.63 & \textbf{1} & 78.89\%  & 92.89\% &  19.00 & 45  & 72.71\% &  87.58\%  \\
%  FocalClick & 4.46 & 2 & 75.59\% & 94.90\%  & 17.74 & 49 & 70.76\% & 88.90\%  \\
%  \rowcolor{gray!20} ISGPC & \textbf{3.36} & \textbf{1} & \textbf{79.43\%} & \textbf{95.11\%}  & \textbf{17.03} & \textbf{44} & \textbf{75.67\%} & \textbf{89.60\%}  \\ 
%  \bottomrule
% \end{NiceTabular}}
% \vspace{-4mm}
% \end{table*}

\begin{table}[t] 
\footnotesize
\caption{Quantitative comparisons on different evaluation metrics, where ResNet50 is adopted as the backbone segmentor. \vspace{-3mm}}
\label{tab:metrics}
\centering
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{1.6mm}{
\begin{NiceTabular}[colortbl-like]{@{}l|cccc@{}}
\toprule \multicolumn{1}{c}{\multirow{2}{*}{Method}} & NoC$_{100}$@90 & NoF$_{100}$@90 & IoU\&1 & IoU\&5    \\ \cmidrule(l){2-5}
 & \multicolumn{4}{c}{Berkeley}  \\ \midrule
  f-BRS-B & 6.21 & 2 & 77.06\% & 85.00\%    \\
 RITM & 3.75 & \textbf{1} & 76.88\% & 94.66\%  \\
 FocusCut & 4.63 & \textbf{1} & 78.89\%  & 92.89\%   \\
 FocalClick & 4.46 & 2 & 75.59\% & 94.90\%  \\
 \rowcolor{gray!20} GPCIS (Ours)  & \textbf{3.36} & \textbf{1} & \textbf{79.43\%} & \textbf{95.11\%}  \\ 
 \midrule
 & \multicolumn{4}{c}{DAVIS} \\ \midrule
   f-BRS-B & 22.62 & 57 & 70.97\% & 83.87\%    \\
 RITM & 18.09 & 51 & 72.89\%  & 89.14\%  \\
 FocusCut & 19.00 & 45  & 72.71\% &  87.58\%   \\
 FocalClick &17.74 & 49 & 70.76\% & 88.90\%   \\
 \rowcolor{gray!20} GPCIS (Ours)   & \textbf{17.03} & \textbf{44} & \textbf{75.67\%} & \textbf{89.60\%} \\ \bottomrule
\end{NiceTabular}}
\vspace{-4mm}
\end{table}


==> misc/tab_metrics2.tex <==

\begin{table*}[t] 
\footnotesize
\caption{Quantitative comparisons on different evaluation metrics, where ResNet50 is adopted as the backbone segmentor. \vspace{-3mm}}
\label{tab:metrics}
\centering
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{1.6mm}{
\begin{NiceTabular}[colortbl-like]{@{}l|cccc@{}}
\toprule \multicolumn{1}{c}{\multirow{2}{*}{Method}} & NoC$_{100}$@90 & NoF$_{100}$@90 & IoU\&1 & IoU\&5    \\ \cmidrule(l){2-5}
 & \multicolumn{4}{c}{Berkeley}  \\ \midrule
  f-BRS-B & 6.21 & 2 & 77.06\% & 85.00\%    \\
 RITM & 3.75 & \textbf{1} & 76.88\% & 94.66\%  \\
 FocusCut & 4.63 & \textbf{1} & 78.89\%  & 92.89\%   \\
 FocalClick & 4.46 & 2 & 75.59\% & 94.90\%  \\
 \rowcolor{gray!20} GPCIS (Ours)  & \textbf{3.36} & \textbf{1} & \textbf{79.43\%} & \textbf{95.11\%}  \\ 
 \midrule
 & \multicolumn{4}{c}{DAVIS} \\ \midrule
   f-BRS-B & 22.62 & 57 & 70.97\% & 83.87\%    \\
 RITM & 18.09 & 51 & 72.89\%  & 89.14\%  \\
 FocusCut & 19.00 & 45  & 72.71\% &  87.58\%   \\
 FocalClick &17.74 & 49 & 70.76\% & 88.90\%   \\
 \rowcolor{gray!20} GPCIS (Ours)   & \textbf{17.03} & \textbf{44} & \textbf{75.67\%} & \textbf{89.60\%} \\ \bottomrule
\end{NiceTabular}}
\vspace{-4mm}
\end{table*}


==> tex/intro.tex <==

\section{Introduction}
\label{sec:intro}

% Recent semantic segmentation models \cite{long2015fully,chen2017deeplab} usually lack the ability to recognize objects in the wild or to respond to the user's interactions for refinement. Therefore, interactive segmentation, which aims to segment the target objects under the user's supervision, has sparked much research interest~\cite{he2014interactive}. Among various types of interaction~\cite{xu2017deep,acuna2018efficient,castrejon2017annotating,ling2019fast,bai2014error,wu2014milcut,majumder2020two,zhang2020interactive}, we focus on the mainstream click-based interactive segmentation, where positive clicks are clicked on the target objects while negative ones are clicked in the incorrectly predicted background region~\cite{jang2019interactive,sofiiuk2020f,sofiiuk2021reviving}. Since the task has practical values for industrial applications, our purpose is to use as few clicks as possible to segment the object with high efficiency.

Driven by the huge potential in reducing the pixel-wise annotation cost, interactive segmentation (IS) has sparked much research interest~\cite{he2014interactive}, which aims to segment the target objects under the user's supervision with less interaction cost and higher efficiency. Among various types of user interaction~\cite{xu2017deep,acuna2018efficient,castrejon2017annotating,ling2019fast,bai2014error,wu2014milcut,majumder2020two,zhang2020interactive}, the click-based mode is the mainstream due to its simplicity, where positive clicks are clicked on the target object while negative ones are clicked in the background regions~\cite{jang2019interactive,sofiiuk2020f,sofiiuk2021reviving}.
In this paper, we aim to accomplish the accurate segmentation of target objects with fewer clicks and faster speed.


% Since the task has practical values for industrial applications, our purpose is to use as few clicks as possible to segment the object with high efficiency.
\input{CVPR_GPIS/misc/fig_first.tex}

% Existing methods can be divided into two completely different categories, bounded by the emergence of deep learning (DL) \cite{lecun2015deep}. The traditional methods \cite{grady2006random,gulshan2010geodesic,kim2010nonparametric,rother2004grabcut}, although equipped with appealing theories and interpretable algorithms, can hardly achieve satisfactory segmentation results because they only utilize the RGB values as image features. In contrast, the DL-based methods encode user supervision as click maps~\cite{xu2016deep,sofiiuk2021reviving}, which are input to the deep neural networks (DNNs) together with the images (and previous prediction masks). However, these methods mainly follow the conventional pipeline of general semantic segmentation models and directly perform pixel-wise classification of the deep features. The classification procedure performed on each pixel individually does not fully utilize the relations between different pixels, especially the clicked pixels. Another critical issue of these methods is that they cannot provide theoretical guarantees that the regions of the clicks can be correctly classified. Although several methods, \eg BRS \cite{jang2019interactive}, f-BRS \cite{sofiiuk2020f}, have been proposed to address this issue via backpropagating refinement scheme, they still lack interpretability and suffer from inefficiency since they require fine-tuning during inference. In this paper, we break out of the framework of current DL-based methods and seek to build a more \textit{efficient} and \textit{elegant} model to \hypertarget{R1}{\dcircle{1}} propagate information from click points to other pixels to encourage correct classification of pixels similar to the clicks or largely distinct from them; \hypertarget{R2}{\dcircle{2}}  make correct predictions at the click points with a high probability.

Against this click-based interactive segmentation task, traditional methods generally utilize the color information of the to-be-segmented images as the features for segmentation~\cite{grady2006random,gulshan2010geodesic,kim2010nonparametric,rother2004grabcut}. Albeit possessing appealing theories and good interpretability, these approaches can hardly achieve satisfactory segmentation performance due to the inadequate exploitation of the image priors from large datasets. Besides, these methods are usually time-consuming because of the involved complicated iterative process. 


With the rapid development of deep learning (DL), recent years have witnessed the promising performance of DL-based methods in this IS task. The most commonly-adopted research line is that the user interaction is encoded as click maps and fed into a deep neural network (DNN) together with input images to extract deep features for the subsequent segmentation~\cite{xu2016deep,sofiiuk2021reviving}. These methods generally suffer from two limitations: 
%1) They generally follow the off-the-shelf pipeline of the semantic segmentation models~\cite{long2015fully,chen2017deeplab} without specific designs for the interactive task. %, and they perform pixel-wise classification individually on the extracted deep features without fully utilizing the relations between different pixels, especially the clicked pixels; 
1) They mainly adopt the off-the-shelf pipeline of the semantic segmentation models and directly perform the pixel-wise classification on the extracted features without specific designs for the IS task, as shown in Fig. \ref{fig:first} (a). As a result, during classification, the deep features corresponding to different pixels are not fully interactive and the information contained in click points can hardly propagate to other pixels;
%Unaware of whether the pixel feature belongs to a clicked point or not, they could possibly output incorrect predictions at clicked pixels \cite{jang2019interactive}. 
%Although the existing BRS \cite{jang2019interactive} and f-BRS \cite{sofiiuk2020f} have the capability to mitigate this issue via backpropagating refinement scheme, such implicit and heuristic design leads to weak interpretability, and the involved fine-tuning mechanism during inference would adversely impair the efficiency.
% 2) There are no explicit theoretical guarantees that the clicked regions can be correctly classified. 
% 2) The pixel features are not fully interactive and the information propagation procedure lacks interpretability. 
 2) There are no explicit theoretical guarantees that the clicked regions can be properly activated and correctly classified. 
% Although existing methods have explored to mitigate these issues via the backpropagating refinement scheme \cite{jang2019interactive,sofiiuk2020f} or the self-attention mechanism \cite{chen2021conditional}, they mainly rely on heuristic designs with weak interpretability, and suffer from unsatisfying inference efficiency or extra computational burden. 
Although the existing CDNet \cite{chen2021conditional} promotes the information propagation from clicks to other pixels via a self-attention mechanism and two diffusion modules, it introduces extra computational burden and still cannot handle the second issue. BRS \cite{jang2019interactive} and f-BRS \cite{sofiiuk2020f} adopt the backpropagating refinement scheme for helping the correct predictions at clicks. However, the design is heuristic with weak interpretability and the involved fine-tuning procedure would adversely impair the efficiency. To alleviate these issues, in this paper, {\textit{we try to jump out of the current DL framework and seek to build a more interpretable and efficient model for the IS task with specific characteristics: \hypertarget{R1}{\dcircle{1}} For each image, the relations between deep features of pixels can be finely and explicitly modeled so that the information contained in clicked pixels can be more effectively propagated to other pixels to promote better segmentation results. 
\hypertarget{R2}{\dcircle{2}} The predictions at clicks are correct with a high probability under better theoretical support.}}
% To build a model that meets our requirements, we suggest taking an alternative view of the interactive segmentation problem: a pixel-level binary classification task on each image, regarding the clicks as training pixels with labels, and the others as testing pixels to be classified into foreground/background classes. Although almost all traditional classification models can handle such binary classification tasks, they mostly require iterative training which hinders efficiency. We suggest that Gaussian process (GP) models \cite{williams2006gaussian} are perfectly qualified for our requirements. GP models are flexible non-parametric models that have straightforward training and inference procedures. They can behave well with only a few training data by utilizing the embedded function priors and the relations between data points (\myhyperlink{R1}{\dcircle{1}}). Furthermore, the training data can be well interpolated (\myhyperlink{R2}{\dcircle{2}}) while uncertainty information can be provided. These advantages are all appealing to interactive segmentation. Besides, deep kernel learning (DKL) \cite{wilson2016deep,wilson2016stochastic} has been proposed to build GP models upon the deep features of data, indicating the adaptability of GP with DNN backbones. % it becomes natural to leverage Gaussian Process (GP) models to solve the micro-level tasks, with reasons from four aspects: (1) The training and inference procedures of GP models (for each image) are straightforward and do not require excessive training over the training data (pixels); (2) For interactive segmentation, there are only a few clicks as training data, which avoids the annoying training complexity of GP models; (3) GP models are flexible non-parametric models that behave well by utilizing the relations between data points, which is appealing to interactive segmentation; (4) The correctness of the clicked positions can be assured.
% %We solve the abovementioned issue by treating IS as a gaussian process classification problem. Specifically, ...
 %formulate the interactive segmentation problem as a pixel-level binary classification task on each image, where the clicked points are regarded as training pixels with labels, \emph{i.e.}, foreground or background, and the unclicked points are taken as the to-be-classified testing pixels.

% suggest taking an alternative view of the interactive segmentation problem: a pixel-level binary classification task on each image, regarding the clicks as training pixels with labels, and the others as testing pixels to be classified into foreground/background classes. 
To this end, we propose to treat the IS problem from an alternative perspective and reformulate it as a pixel-level binary classification task on each image, where clicks are viewed as training pixels with classification labels, \emph{i.e.}, foreground or background, and the unclicked points as the to-be-classified testing pixels, as shown in Fig.~\ref{fig:first}~(b). Based on such a setting, Gaussian process (GP)~\cite{williams2006gaussian} is a suitable tool for building the model with the aforementioned functionalities we expect, due to its intrinsic properties: 
% 1) GP explicitly measures the relations between training data and testing data via kernel function and it can perform well with only a small amount of training clicks;
1) As a non-parametric model, GP explicitly measures the relations between data via a kernel function and can perform well with only a small number of training clicks;
2) The training data can be well interpolated, benefitting correct predictions at clicked points; 3) GP has straightforward training/inference procedures without iterative optimization steps. However, it is infeasible to directly apply the GP tool to the binary classification task. Firstly, GP posterior is intractable in the classification task. Besides, the computation cost in conventional GP models is cubic w.r.t. the number of data points, which is unfriendly for efficient interaction. 


%% put below.
% Besides, 
% These advantages are all appealing to interactive segmentation. Besides, deep kernel learning (DKL) \cite{wilson2016deep,wilson2016stochastic} has been proposed to build GP models upon the deep features of data, indicating the adaptability of GP with DNN backbones. 



% it becomes natural to leverage Gaussian Process (GP) models to solve the micro-level tasks, with reasons from four aspects: (1) The training and inference procedures of GP models (for each image) are straightforward and do not require excessive training over the training data (pixels); (2) For interactive segmentation, there are only a few clicks as training data, which avoids the annoying training complexity of GP models; (3) GP models are flexible non-parametric models that behave well by utilizing the relations between data points, which is appealing to interactive segmentation; (4) The correctness of the clicked positions can be assured.
%We solve the abovementioned issue by treating IS as a gaussian process classification problem. Specifically, ...


% Despite the benefits of GP models discussed above, there are still two main obstacles to applying GP models to interactive segmentation. On one hand, when applied to classification tasks, GP encounters intractable posterior which needs to be approximated. On the other hand, GP models inherently suffer from scalability issues since the computation cost of training/inference is cubic with the number of training/testing data. Fortunately, in interactive segmentation, the number of clicks (training pixels) is always small, thus only the inference complexity needs to be reduced. 



% We propose Interactive Segmentation as Gaussian Process Classification (GPCIS) by introducing GP models to DL-based methods while addressing the above-mentioned issues. Firstly, to build a GP classification model without impeding efficiency, we utilize amortized variational inference \cite{kingma2013auto} to approximate the intractable GP posterior. Secondly, we make use of the latest techniques \cite{wilson2020efficiently,wilson2021pathwise} for efficient sampling of GP posterior, without sacrificing the interpolation accuracy on the training pixels. The inference complexity is thus reduced from cubic to linear with the number of testing pixels. Furthermore, we extend the ideas of DKL to training kernel hyperparameters in both function space and weight space end-to-end with the DNN parameters, to achieve full flexibility of the model.

% Our contributions can be concluded as follows: (1) We develop a new perspective for interactive segmentation and build an interpretable model to propagate information from the clicks and guarantees the correct predictions at click points with a high probability; (2) To the best of our knowledge, we are the first to apply deep kernel learning methods with the efficient decoupled posterior sampling techniques to computer vision tasks, which is inspiring for other applications; (2) We achieve the state-of-the-art experimental results on various interactive segmentation benchmarks with little extra computational burden.



To address these aforementioned issues, in this paper, we carefully formulate the interactive segmentation task as a Gaussian process classification model and propose a general framework with competitive inference efficiency, which has good application potential for practical interactive segmentation. Our contributions are mainly summarized as:

%Novel Formulation
\noindent \textbf{1)} We rethink the IS task and step out of the current research framework. Specifically, we creatively propose to regard it as a pixel-wise binary classification on each input image and then construct the corresponding GP classification model. %To the best of our knowledge, we are the first to integrate the classic GP model into the IS task.

% Efficient GP Inference
\noindent \textbf{2)} To adapt the GP model to the IS task, we propose to utilize amortized variational inference to efficiently approximate the intractable GP posterior, and then reduce its sampling complexity from cubic to linear using the modern techniques of decoupled GP posterior \cite{wilson2020efficiently,wilson2021pathwise}. To improve learning flexibility, we extend deep kernel learning to both terms of our decoupled GP posterior sampling framework. %Such treatment is also inspiring to other potential applications of GP models.


\noindent \textbf{3)} By seamlessly integrating the derived GP posterior sampling method with DNN backbones, we construct an interpretable framework, where every computation step has clear physical meanings,
which provides explicit modeling of correlations of pixels as well as theoretical support for correct predictions at clicked points.%Based on the derived GP posterior sampling method, we correspondingly construct the framework, where every computation step has clear physical meanings.

% To improve the learning flexibility, we further embed the double space deep kernel learning strategy into the framework. 


% \textcolor{red}{The main specificity of GPCIS is 1) From Fig.~\ref{fig:first}~(b), under the explicit guidance of GP posterior, the information at clicks can finely propagate to the entire image and boost the segmentation results; 2) The correctness of predictions at clicks has good theoretical guarantees.}

%  Satisfactory Performance
\noindent \textbf{4)} Extensive experimental comparisons as well as model verification comprehensively substantiate the superiority of our proposed method in segmentation quality, computation cost, and inference speed. Our method can consistently achieve superior performance under different backbone segmentors, showing fine generality. %Additionally, the effectiveness of our proposed modules is fully validated through ablation studies.




% We propose Interactive Segmentation as Gaussian Process Classification (GPCIS) by introducing GP models to DL-based methods while addressing the above-mentioned issues. Firstly, to build a GP classification model without impeding efficiency, we utilize amortized variational inference \cite{kingma2013auto} to approximate the intractable GP posterior. Secondly, we make use of the latest techniques \cite{wilson2020efficiently,wilson2021pathwise} for efficient sampling of GP posterior, without sacrificing the interpolation accuracy on the training pixels. The inference complexity is thus reduced from cubic to linear with the number of testing pixels. Furthermore, we extend the ideas of deep kernel learning (DKL) \cite{wilson2016deep,wilson2016stochastic} to training kernel hyperparameters in both function space and weight space end-to-end with the DNN parameters, to achieve full flexibility of the model.

% Our contributions can be concluded as follows: (1) We develop a new perspective for interactive segmentation and build an interpretable model to propagate information from the clicks and guarantees the correct predictions at click points with a high probability; (2) To the best of our knowledge, we are the first to apply deep kernel learning methods with the efficient decoupled posterior sampling techniques to computer vision tasks, which is inspiring for other applications; (3) We achieve the state-of-the-art experimental results on various interactive segmentation benchmarks with little extra computational burden.


